Horseshoes for singly thermostated hamiltonians

This note studies 1 and 2 degree of freedom hamiltonian systems that are thermostated by a single-variable thermostat. Under certain conditions on the hamiltonian and thermostat, the existence of a horseshoe in the flow of the thermostated system is proven.

==> nhht-nhim-main-thm-mac.ltx <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,4320.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(849,595){\makebox(0,0)[r]{\strut{}-0.04}}%
      \csname LTb\endcsname%%
      \put(849,1011){\makebox(0,0)[r]{\strut{}-0.02}}%
      \csname LTb\endcsname%%
      \put(849,1427){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%%
      \put(849,1844){\makebox(0,0)[r]{\strut{}0.02}}%
      \csname LTb\endcsname%%
      \put(849,2260){\makebox(0,0)[r]{\strut{}0.04}}%
      \csname LTb\endcsname%%
      \put(849,2676){\makebox(0,0)[r]{\strut{}0.06}}%
      \csname LTb\endcsname%%
      \put(849,3092){\makebox(0,0)[r]{\strut{}0.08}}%
      \csname LTb\endcsname%%
      \put(849,3509){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%%
      \put(849,3925){\makebox(0,0)[r]{\strut{}0.12}}%
      \csname LTb\endcsname%%
      \put(951,409){\makebox(0,0){\strut{}-10}}%
      \csname LTb\endcsname%%
      \put(2413,409){\makebox(0,0){\strut{}-5}}%
      \csname LTb\endcsname%%
      \put(3876,409){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%%
      \put(5338,409){\makebox(0,0){\strut{}5}}%
      \csname LTb\endcsname%%
      \put(6800,409){\makebox(0,0){\strut{}10}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(153,2364){\rotatebox{-270}{\makebox(0,0){\strut{}$\fouriertransform{p ²}$}}}%
      \csname LTb\endcsname%%
      \put(7004,2364){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(3875,130){\makebox(0,0){\strut{}$ ω $}}%
      \csname LTb\endcsname%%
      \put(3875,4040){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(3875,4133){\makebox(0,0){\strut{}}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(4636,2780){\makebox(0,0)[l]{\strut{}$k=6, n=1$}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(4636,3301){\makebox(0,0)[l]{\strut{}$k=5, n=4/3$}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(4636,3509){\makebox(0,0)[l]{\strut{}$k=4, n=2$}}%
      \colorrgb{0.00,0.00,0.00}%%
      \put(4636,3821){\makebox(0,0)[l]{\strut{}$k=3, n=4$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{nhht-nhim-main-thm-mac}}%
    \gplfronttext
  \end{picture}%
\endgroup

